Riemannian Score-Based Generative Modelling

Score-based generative models (SGMs) are a powerful class of generative models that exhibit remarkable empirical performance. Score-based generative modelling (SGM) consists of a ``noising'' stage, whereby a diffusion is used to gradually add Gaussian noise to data, and a generative model, which entails a ``denoising'' process defined by approximating the time-reversal of the diffusion. Existing SGMs assume that data is supported on a Euclidean space, i.e. a manifold with flat geometry. In many domains such as robotics, geoscience or protein modelling, data is often naturally described by distributions living on Riemannian manifolds and current SGM techniques are not appropriate. We introduce here Riemannian Score-based Generative Models (RSGMs), a class of generative models extending SGMs to Riemannian manifolds. We demonstrate our approach on a variety of manifolds, and in particular with earth and climate science spherical data.

==> diff_nf_sde.tex <==
    \section{Difference between ODE and SDE likelihood computations}
    \label{sec:diff-betw-ode}
    
    In this section, we show that the likelihood computation from
    \cite{song2020score} does not coincide with the likelihood computation
    obtained with the SDE model. We present our findings in the Riemannian setting
    but our results can be adapted to the Euclidean setting with arbitrary
    forward dynamics. Recall that we consider a Brownian motion on the manifold as a forward process
    $(\bfB_t^\M)_{t \in \ccint{0,T}}$ with $(p_t)_{t \in \ccint{0,T}}$ the associated family
    of densities. We have that for any $t \in \ccint{0,T}$ and $x \in \M$
    \begin{equation}
      \label{eq:forward}
      \partial_t p_t(x) = \tfrac{1}{2} \Delta_\M p_t(x) = \dive(\tfrac{1}{2}p_t \nabla \log p_t )(x)  . 
    \end{equation}
    
    
    \paragraph{ODE model.}
    In the case of the ODE model, we define $(\bfX_t)_{t \in \ccint{0,T}}$ such that
    $\bfX_0 \sim p_0$ and satisfies
    $\rmd \bfX_t = -\tfrac{1}{2}  \nabla \log p_t(\bfX_t) \rmd t$. The family of densities $(q_t)_{t \in \ccint{0,T}}$ associated with $(\bfX_t)_{t \in \ccint{0,T}}$ also
    satisfies \eqref{eq:forward}. Now consider
    $(\bfhX_t)_{t \in \ccint{0,T}} = (\bfX_{T-t})_{t \in \ccint{0,T}}$, this satisfies $\bfhX_0 \sim p_T$ with 
    \begin{equation}
      \label{eq:backward_flow_appendix}
     \rmd \bfhX_t = \tfrac{1}{2}  \nabla \log p_{T-t}(\bfhX_t) \rmd t  .
    \end{equation}
    Finally, we consider $(\bfY_t^{\mathrm{ODE}})_{t \in \ccint{0,T}}$ which also satisfies
    \cref{eq:backward_flow_appendix} and such that $\bfY_0^{\mathrm{ODE}}\sim \piinv$. Denoting
    $(q_t^{\mathrm{ODE}})_{t \in \ccint{0,T}}$ the densities of
    $(\bfY_t^{\mathrm{ODE}})_{t \in \ccint{0,T}}$ w.r.t. $\piinv$ we have for any $t \in \ccint{0,T}$ and $x \in \M$
    \begin{equation}
      \label{eq:proba_flow_ode}
     \partial_t q_t^{\mathrm{ODE}}(x) =  -\dive( \tfrac{1}{2} q_t^{\mathrm{ODE}} \nabla\log p_{T-t} )(x)  . 
    \end{equation}
    
    \paragraph{SDE model.}
    When sampling we consider a process $(\bfY^{\mathrm{SDE}}_t)_{t \in \ccint{0,T}}$ such that
    $\bfY^{\mathrm{SDE}}_0$ has distribution $\piinv$ and whose family of densities
    h$(q_t^{\mathrm{SDE}})_{t \in \ccint{0,T}}$ satisfies for any $t \in \ccint{0,T}$ and $x \in \M$
    \begin{equation}
      \label{eq:proba_flow_sde}
      \partial_t q_t^{\mathrm{SDE}}(x) = -\dive(\nabla \log p_{T-t} q_t^{\mathrm{SDE}}(x)) +\tfrac{1}{2}\Delta_\M q_t^{\mathrm{SDE}}(x) =- \dive(q_t^{\mathrm{SDE}}\{\nabla\log p_{T-t} - \tfrac{1}{2}\nabla\log q_t^{\mathrm{SDE}}\})(x)  . 
    \end{equation}
    Hence, \cref{eq:proba_flow_ode} and \cref{eq:proba_flow_sde} do not agree,
    except if $q_t^{\mathrm{SDE}} = q_t^{\mathrm{ODE}} = p_{T-t}$ which is the case if and only if $\bfY^{\mathrm{SDE}}_0$ and
    $\bfY_0^{\mathrm{ODE}}$ have the same distribution as $\bfX_T$. Note that it is possible to
    evaluate the likelihood of the SDE model using that
    \begin{equation}
      \partial_t \log q_t^{\mathrm{SDE}}(\bfY^{\mathrm{SDE}}_t) = \big\{\nabla\log p_{T-t}(\bfY^{\mathrm{SDE}}_t) -\tfrac{1}{2}\nabla\log q_t^{\mathrm{SDE}}(\bfY^{\mathrm{SDE}}_t) \big\}\rmd t  . 
    \end{equation}
    We can use the score approximation $\bm{s}_\theta(t,x)$ to approximate
    $\nabla \log p_t(x)$ for any $t \in \ccint{0,T}$ and $x \in \M$. In order to
    approximate $\nabla \log q_t^{\mathrm{SDE}}$, one can consider another neural network
    $\bm{t}_\theta(t,x)$ approximating $\nabla \log q_t^{\mathrm{SDE}}(x)$ for any $t \in \ccint{0,T}$
    and $x \in \M$. This approximation can be obtained using the implicit score loss
    presented in \Cref{sec:riem-score-appr}.
    
    
    %%% Local Variables:
    %%% mode: latex
    %%% TeX-master: "main"
    %%% End:

